Arithmetic Feature Interaction Is Necessary for Deep Tabular Learning

Until recently, the question of the effective inductive bias of deep models on tabular data has remained unanswered. This paper investigates the hypothesis that arithmetic feature interaction is necessary for deep tabular learning. To test this point, we create a synthetic tabular dataset with a mild feature interaction assumption and examine a modified transformer architecture enabling arithmetical feature interactions, referred to as AMFormer. Results show that AMFormer outperforms strong counterparts in fine-grained tabular data modeling, data efficiency in training, and generalization. This is attributed to its parallel additive and multiplicative attention operators and prompt-based optimization, which facilitate the separation of tabular samples in an extended space with arithmetically-engineered features. Our extensive experiments on real-world data also validate the consistent effectiveness, efficiency, and rationale of AMFormer, suggesting it has established a strong inductive bias for deep learning on tabular data. Code is available at https://github.com/aigc-apps/AMFormer.

==> sec/rebuttal.tex <==
\textit{We are truly grateful for the recognition and positive feedback received from all reviewers regarding the novelty, significance, technical designs, evaluation, and overall presentation of our work (with the exception of Section~4 we admit). The comments provided by the reviewers have been both inspiring and helpful, guiding us in enhancing our work. We have provided detailed responses to each comment below.}

\section{Response to Reviewer \#1}


\noindent\textbf{W1. Impacts of other feature interaction types.}
In the experiments, we conducted empirical analyses of alternative feature interactions. We compared our method with recently proposed crossing-based (DCN-V2 and DCAP) and Transformer-based (AutoInt and FT-Trans.) interactions. Additionally, we compared our complete arithmetic feature interaction with additive-only and multiplicative-only ones in the ablation study. The results confirm that explicit and complete arithmetic feature interaction is the most effective. A more detailed discussion will be provided in the final version. Thank you for your comment.

\noindent\textbf{W2. Representative datasets.}
Due to page constraints, we only provided a concise description of the datasets used in Section 5.1. We will include all the necessary information of data in the Appendix. 
For the ablation study, we report the results on the EP and MI data due to the same limitation. We selected these two as they have the largest number of features and represent both classification and regression tasks (para. 1, left, page 7). Further results on parameter sensitivity can be found in the Appendix.

\noindent\textbf{Q1. DCAP has competitive performance in dataset HC but worse performance in other datasets.}
While it is challenging to provide a precise explanation, we speculate that it is likely because of the presence of categorical features in HC and the nature of the home credit default risk prediction task. These factors require the exploration of deep and meaningful interactions, which the Transformer architecture and the crossing interaction design of DCAP excel at. This is corroborated by the good performance of the other two Transformer-based methods on the HC dataset. Although the advantage of DCAP may not be as pronounced on other datasets, it still performs well. In fact, DCAP achieves the highest overall ranking among all tested baselines.

%It is difficult for us to precisely explain why DCAP performs well, but we speculate it may be due to the presence of categorical features in HC, which relies more on mining deep interactions. Therefore, the transformer in DCAP, along with cross-interactions, can lead to more complex interactions. At the same time, we also observed that AutoInt and FT-Transformer perform well on this dataset because of utilizing transformer.

\noindent\textbf{Q2. open-source code.}
Yes, we will share our code, data, and experimental settings openly. Our aim is to make it possible for others to replicate our work with ease.










\section{Response to Reviewer \#3}


\noindent\textbf{W1. More challenge demonstrations.}
Thank you for the valuable suggestion. We will incorporate case studies in Secs. 3\&5 to enhance clarity and comprehensibility.

% This suggestion is excellent, and we will consider conducting some case studies, in Section 3 and Section 5, to make the method more intuitive and easier to understand.

\noindent\textbf{W2. Grammatical mistakes and typos.}
We will thoroughly proofread our paper again. Thanks.
%trying our best to correct the grammatical mistakes and typos. 
% We will review our paper again for grammar and spelling errors and make the necessary corrections before the final version.

\noindent\textbf{W3\&Q1. Symbol definition.}
Thank you for your suggestions. In the next version, we will provide clearer symbol definitions, include a summary, and correct any incorrect terminology usage. 
% Thank you very much for your suggestions. In the subsequent version, we will introduce clearer symbol definitions, present a summary, and rectify incorrect terminology usage.

\noindent\textbf{Q2. Dataset metrics.} 
We adopt the evaluation metrics used in previous studies for each dataset. The discrepancy in metrics between the two binary classification datasets is due to the differing balance of positive and negative examples. It's important to note that the EP dataset has balanced samples, while the HC dataset is highly imbalanced with a ratio of around 
% \colorbox{red}{
1:10 for positive to negative examples. Therefore, we use Acc for EP, but it may not be suitable for HC. In this case, AUC is a better choice. In Table~1, the terms `\# Num.' and `\# Cate.' represent the numbers of numerical and categorical features, respectively. We will include all of these details in our paper. Thank you!


%In previous studies, the HC dataset is imbalanced, so AUC was used to evaluate performance, whereas the EP dataset does not have this issue, so ACC is employed. We followed this setup in our paper. In the final version, we will provide explanations for \# Num. and \# Cate., which represent numerical features and categorical features, respectively.



\section{Response to Reviewer \#4}

\noindent\textbf{W1\&Q2--Q4. Presentation of the method.}
We apologize for the clarity issues in the methodology section. We will reorganize and rephrase the section to enhance the readability.

First, $S$ represents the similarity matrix obtained from the log-transformed query and key in the multiplicative interaction: $S = Q_{log} \cdot K_{log}^T$.
%
$R_A$ and $R_P$ represent the outputs of additive and multiplicative interactions, respectively. Specifically, $R_A = Attention(Q,K,V)$ is derived with standard attention calculation except that we use prompt embeddings as the query.
The computation of $R_P$ is slightly more complex. We introduce a Top-K operator to address numerical issues and ensure stability during the multiplication interaction. Firstly, we calculate the similarity matrix $S$ as mentioned earlier. Then, we use the Top-K operator to identify the top-k most relevant items for each query/prompt in $Q_{log}$. From these top-k items, we consider the log-transformed values in $V_{log}$ and perform a weighted sum followed by an exponential operation to obtain the final result, $R_P$. The process is illustrated in Figure 2.

To address the computational complexity issue, we introduced a prompt optimization strategy, which replaces the QK-similarity with PK-similarity. The result of PK-similarity is represented as $S_P$.


\noindent\textbf{W2\&Q6. Compare with GAM-based methods.}
GAMs are known for their focus on model interpretability, but often face a trade-off with performance, leading to reduced effectiveness. Taking the SIAN method for instances, DNN and tree models outperformed SIAN in many cases, weakening its position as a strong baseline. Consequently, we exclude the comparison with GAM-based methods. We hope you could understand our choice.

%However, for the sake of completeness, we will consider including these results in the Appendix.

% GAMs emphasize on model interpretability, and there is usually a trade-off between performance and interpretability, often resulting in a decrease in effectiveness. In the SIAN paper, NODE-GA$^2$M and DNN models outperformed SIAN in many cases, which makes SIAN not a strong baseline. Therefore, in this version of the paper, we did not include the results of GAM-based methods. For the sake of completeness, we will consider incorporating this section in future versions.

\noindent\textbf{Q1. Sparsity in synthetic dataset.}
Our synthetic data is dense in terms of features, and we refer to the feature interactions as `sparse'. This means that, on average, each interaction involves four features, and we anticipate this number to remain consistent as the total number of features increases. We apologize for any confusion caused and will provide further clarification to avoid misunderstandings.

%Our writing in this section is a bit confusing. In the synthetic dataset, sparsity refers to the fact that there is a 50\% probability that a feature's order will be 0, meaning there is sparsity in the multiplication interactions between features (as described in \textbf{Data construction} in Section 3).

\noindent\textbf{Q5. Learned multiplicative interaction or prior knowledge.}
Our model learns the multiplicative interaction groups, ensuring a fair comparison.
When we mention `constant rules', we are referring some patterns ingrained in the prompt parameters, as opposed to being solely data-dependent with classic Transformer. We will revise this part for clarification. Thank you for bringing it to our attention.


%The multiplication interactions mentioned in our paper are not prior knowledge, and we did not leak information to the model about how features should interact. During the training, interactions are introduced through prompt tokens, making our approach not purely data-dependent compared to other transformer models.


% The term "constant rule" mentioned here refers to the idea that a model can learn a fixed interaction, such as calculating BMI from height and weight using multiplication and division. The goal is to make the model learn this interaction logic rather than directly using the equation $height / weight^2$ to create an additional feature for the model. Therefore, we conducted fair experiments and did not leak any prior knowledge to our method.

